Doing good by fighting fraud: Ethical anti-fraud systems for mobile payments

App builders commonly use security challenges, a form of step-up authentication, to add security to their apps. However, the ethical implications of this type of architecture has not been studied previously. In this paper, we present a large-scale measurement study of running an existing anti-fraud security challenge, Boxer, in real apps running on mobile devices. We find that although Boxer does work well overall, it is unable to scan effectively on devices that run its machine learning models at less than one frame per second (FPS), blocking users who use inexpensive devices. With the insights from our study, we design Daredevil, anew anti-fraud system for scanning payment cards that work swell across the broad range of performance characteristics and hardware configurations found on modern mobile devices. Daredevil reduces the number of devices that run at less than one FPS by an order of magnitude compared to Boxer, providing a more equitable system for fighting fraud. In total, we collect data from 5,085,444 real devices spread across 496 real apps running production software and interacting with real users.

==> duppy <==
#!/usr/bin/env perl
 
# Finds duplicate adjacent words.
 
use strict ;
 
my $DupCount = 0 ;
 
if (!@ARGV) {
  print "usage: dups <file> ...\n" ;
  exit ;
}
 
while (1) {
  my $FileName = shift @ARGV ;
 
  # Exit code = number of duplicates found.  
  exit $DupCount if (!$FileName) ;
 
  open FILE, $FileName or die $!; 
   
  my $LastWord = "" ;
  my $LineNum = 0 ;
   
  while (<FILE>) {
    chomp ;
 
    $LineNum ++ ;
     
    my @words = split (/(\W+)/) ;
     
    foreach my $word (@words) {
      # Skip spaces:
      next if $word =~ /^\s*$/ ;
 
      # Skip punctuation:
      if ($word =~ /^\W+$/) {
        $LastWord = "" ;
        next ;
      }
       
      # Found a dup? 
      if (lc($word) eq lc($LastWord)) {
        print "$FileName:$LineNum $word\n" ;
        $DupCount ++ ;
      } 
 
      # Mark this as the last word:
      $LastWord = $word ;
    }
  }
   
  close FILE ;
}


==> goals.tex <==
\section{Goals}
This paper describes \system, a system that enables seamless scanning and
verification of payment cards. We have four goals for the system.

\textbf{Correctness}
Incorrect scanning of a legitimate payment card leads to rejection of a
valid payment method. Inconsistent fraud checks leads to false positives.
In either case, a good user is denied the use of a service, through no fault
of their own. Ensuring correctness also reduces the false negatives. A high false
negative rate is an ineffective deterrent against fraud. To aid our ability to make
correct decisions, we strive to maximally utilize the data stream obtained from the
camera. This provides a way for us to obtain more predictions, thereby increasing
the odds of making a correct prediction. Additionally, the challenges within \system
contain some overlap, serving as a redundancy check for validating our predictions.

\textbf{Speed}
Security should not come at the cost of usability. Slow verification leads to blocking
of good users, since users turn away if the verification takes too long. From our production
deployment, we observe that users give up if the scanning takes more than 20s. We
speed up our verification through algorithmic improvements to our machine learning design
and manufacture avenues for data and task level parallelism.

\textbf{Ethical}
We believe it is unfair for a user on a low-end phone to incur a significant time to
verify themselves as opposed to a user on a high-end phone. More importantly, we want
to make sure that users on all phones are able to easily verify themselves without being
blocked. Our design choices to ensure the goals of correctness and speed were informed by
our goal to be ethical.

\textbf{Privacy Preservation}
We want to minimize avenues for user data breach which facilitates card-not-present fraud
in the first place. This requires that we do not send the user data to our servers, pushing
bulk of the processing to the client. Additionally, machine learning models have been shown
to leak information about their training data. To alleviate this concern, we train our machine
learning models with realistic fake data generated by our novel automated credit card image
generation system, Mystique.


==> motivating_example.tex <==


\section{Motivation: Ethical fraud challenges}
This story, based on our experiences, illustrates the difficulties of
preventing fraud. Apps need to be smart about how they block
transactions and even if they are doing right by their business their
fraud techniques might be unethical, and there is \emph{not} an easy
way around it.

Milo is a drug dealer. As his criminal enterprise grows beyond his
local neighborhood, he needs to find new distribution mechanisms to
move drugs around the city. Since most of Milo's employees don't
drive, Milo turns to an up-and-coming ride sharing company, Flip, to
do his drug runs \cite{uber_drug_runs}. However, given the number of
rides Milo's team needs to do, paying for them would be cost
prohibitive. Instead, Milo buys stolen credit card numbers and uses
them to pay for his drug runs \cite{buy_stolen_cc}. Since Flip is a
relatively new company and has not had to deal with fraud, they have
few defenses and Milo and his crew rack up a huge bill paid for using
stolen credit cards. The scheme works so well, Milo tells his friends
in other cities about it, and now Flip is a major source of
transportation for the underground drug trade.

When Flip allows a ride to happen that Milo and his crew pay for using
stolen card numbers, eventually the rightful card owner disputes these
charges with their bank, which results in a chargeback. Chargebacks
are particularly devastating for Flip because banks claw back the
money that they had collected and they charge an additional dispute
fee, which can be as much as \$15 per chargeback
\cite{stripe_disputes}. Thus, banks use chargebacks to incentivize
financially Flip (and any apps that accept payments) to reduce
fraud. Unfortunately, the scale of fraud is so high that it is
beginning to threaten Flip's growing business.

Flip hires Annie, a machine learning expert to come up with a technique
for predicting fraudulent rides before they happen to stop them. Annie
acts quickly and uses signals, including the zip code of the ride, to
train a machine learning model to predict fraud. Her model works well,
and she blocks almost all of Milo's ride requests before the ride
happens, which stops most of the fraud \cite{Stein11, botmaker}.

Annie digs into the overall impact of her anti-fraud algorithm,
evaluating both, the impact on fraud as well as the lost revenue due
to blocking transactions for otherwise good users accidentally flagged
(false positives) \cite{airbnb_false_positive}. She finds that although
her algorithm brings fraud back down to acceptable levels, as many as
50\% of the transactions that her system blocks are false
positives. It turns out that her algorithm was using the zip code as a
key feature to make decisions, so effectively anyone who lives in a
high crime area was unable to use Flip's service \cite{Oneil17},
creating an ethical dilemma for Flip. \textbf{If they stop blocking
  transactions then their service will become too expensive for people
  from a low socioeconomic status to use, but if they keep blocking
  fraud then anyone who lives in a high crime area, including good
  users, is unable to use the service.}

Annie develops a user-facing challenge that empowers users to verify
themselves automatically \cite{lyft_blog}. Annie's challenge lets
users scan their cards to prove that they possess the physical card
\cite{Din20}. The main insight is that fraudsters buy credit card
numbers and not the physical card, but that a legitimate user who owns
a credit card should have the physical card available, making card
scanning easy for good users to pass while continuing to stop
fraud. Her challenge includes cutting-edge machine learning that runs
directly on the device itself to prove possession of the card and
verify that the cards that users scan are genuine credit cards. She
deployed this challenge and recovered 60\% of the people that blocking
alone would have otherwise prevented from using the service. However,
as she digs deeper, she notices that most of the 40\% of false
positives that are unable to pass the challenge live in low-income
areas. It turns out that Annie's machine learning algorithms work
great on high-end and mid-range devices, but simply do not work on
low-end phones. \textbf{Thus, despite having a massive positive impact
  on the Flip business, they are still blocking people of a low
  socioeconomic status who disproportionately use low-end phones.}

Our goal is to define the principles of how apps can use cutting-edge
machine learning on mobile devices despite the vastly different
performance characteristics of devices that one is likely to see in
practice. In other words, we strive to show how to design and
implement ethical fraud challenges.


==> passive <==
#!/bin/bash
 
irregulars="awoken|\
been|born|beat|\
become|begun|bent|\
beset|bet|bid|\
bidden|bound|bitten|\
bled|blown|broken|\
bred|brought|broadcast|\
built|burnt|burst|\
bought|cast|caught|\
chosen|clung|come|\
cost|crept|cut|\
dealt|dug|dived|\
done|drawn|dreamt|\
driven|drunk|eaten|fallen|\
fed|felt|fought|found|\
fit|fled|flung|flown|\
forbidden|forgotten|\
foregone|forgiven|\
forsaken|frozen|\
gotten|given|gone|\
ground|grown|hung|\
heard|hidden|hit|\
held|hurt|kept|knelt|\
knit|known|laid|led|\
leapt|learnt|left|\
lent|let|lain|lighted|\
lost|made|meant|met|\
misspelt|mistaken|mown|\
overcome|overdone|overtaken|\
overthrown|paid|pled|proven|\
put|quit|read|rid|ridden|\
rung|risen|run|sawn|said|\
seen|sought|sold|sent|\
set|sewn|shaken|shaven|\
shorn|shed|shone|shod|\
shot|shown|shrunk|shut|\
sung|sunk|sat|slept|\
slain|slid|slung|slit|\
smitten|sown|spoken|sped|\
spent|spilt|spun|spit|\
split|spread|sprung|stood|\
stolen|stuck|stung|stunk|\
stridden|struck|strung|\
striven|sworn|swept|\
swollen|swum|swung|taken|\
taught|torn|told|thought|\
thrived|thrown|thrust|\
trodden|understood|upheld|\
upset|woken|worn|woven|\
wed|wept|wound|won|\
withheld|withstood|wrung|\
written"
 
if [ "$1" = "" ]; then
 echo "usage: `basename $0` <file> ..."
 exit
fi
 
egrep -n -i --color \
 "\\b(am|are|were|being|is|been|was|be)\
\\b[ ]*(\w+ed|($irregulars))\\b" $*
 
exit $?


==> threat.tex <==
\section{Threat Model}
\label{sec:threat_model}
We position \system as a payment card verification system to combat
against card-not-present credit card fraud.  In our threat model, 
the attacker acquires stolen credit card information,  such as the
card number (PAN), cardholder’s name, expiration date, billing address
etc. Although the card information available to the attacker is complete
and accurate, the attacker does not have access to the physical card
itself. The attacker’s goal is to authorize transactions with the stolen
information.

We assume that the attacker is using their phone to authorize such
a transaction, and we build our defenses on the phone to collect signals
to verify whether or not the scanned image provided by the user came from
a real, physical card. While orthogonal to our work, researchers have studied
ways to combat  fraud carried out by compromising apps \cite{Din20}, we do not
consider attacks against our app running on the phone.

